Continual and Sliding Window Release for Private Empirical Risk Minimization

It is difficult to continually update private machine learning models with new data while maintaining privacy. Data incur increasing privacy loss -- as measured by differential privacy -- when they are used in repeated computations. In this paper, we describe regularized empirical risk minimization algorithms that continually release models for a recent window of data. One version of the algorithm uses the entire data history to improve the model for the recent window. The second version uses a sliding window of constant size to improve the model, ensuring more relevant models in case of evolving data. The algorithms operate in the framework of stochastic gradient descent. We prove that even with releasing a model at each time-step over an infinite time horizon, the privacy cost of any data point is bounded by a constant $\epsilon$ differential privacy, and the accuracy of the output models are close to optimal. Experiments on MNIST and Arxiv publications data show results consistent with the theory.

==> sections/continual.tex <==
\section{Continual Release}\label{sec:continualrelease}

Algorithm~\ref{alg:continualsampling} provides a solution to the multi-scale release problem while guaranteeing only constant privacy loss over infinite timescales. A potential shortcoming of this method is that, while models representing smaller recent datasets are released at regular intervals, the most `global' model (covering all data up to time $T$) is only updated at exponentially growing time intervals of $B$, $2B$, $4B$, .. $2^kB$. After an appropriate burn-in period, this may be acceptable in an I.I.D. scenario. When the last global model represents a sufficient datasize, there will not be a large expected improvement in performance associated with adding small amounts of new data. Despite this, a potential issue arises in online and streaming scenarios where there is often no guarantee that non-I.I.D behaviour, such as concept drift or distribution shift, will not occur. A natural next step is to ask if we can extend our multi-resolution release algorithm to include the maintenance of an up-to-date global model at all time steps, in the style of \textit{continual release}. 

\myparagraph{Shortcomings of Naive Approaches} Naive approaches to continually releasing private empirical risk minimization algorithms suffer from significant degradation of privacy guarantees over time. For example, suppose we retrain a private empirical risk minimization algorithm each time a new datapoint arrives. Each model is $\epsilon$-differentially private. In this scenario the privacy of datapoints that arrived at the beginning of the data stream degrades to $T\epsilon$ at time $T$. If we instead use a sliding window of the $w$ most recent points for each value of $T\geq w$, then the privacy guarantee degrades to only $w\epsilon$ but at the cost of no longer performing true continual release over the entire existing dataset. Suppose instead that after a burn in period of $t_0$ datapoints we release trained models using constant Laplace noise, in the style of Algorithm~\ref{alg:continualsampling}. The privacy guarantee then degradades to $\epsilon(t_0ln(T)-t_0+1)$.



\subsection{Basic Continual Release Algorithm}

Our approach to continual release uses incoming data to continually update the multi-resolution models previously released by Algorithm~\ref{alg:continualsampling}. We obtain up-to-date fine-tuned models at all time steps, with only constant privacy loss. A biased regularization term ensures the inclusion of global information in the fine-tuned current model by biasing the updated model towards the most recent global model released by Algorithm~\ref{alg:continualsampling}. 

\begin{figure}[h]
    \centering
    \begin{minipage}{.5\textwidth}
        \centering
    \includegraphics[width=\linewidth]{images/continualfig1.png}
    \caption{Model Hierarchy }
    \label{fig:conthierarchy1}
    \end{minipage}%
    \begin{minipage}{0.5\textwidth}
        \centering
          \includegraphics[width=\linewidth]{images/continualfig2.png}
    \caption{Model Hierarchy}
    \label{fig:conthierarchy2}
    \end{minipage}
\end{figure}


Denote the most recent global model by $f_g$, parameterized by weights $\mathbf{w}_g$. This is the model trained at $a_1$ in Figure~\ref{fig:conthierarchy1} using dataset $D^{T'}=\{(\mathbf{x}_t, y_t):t\in[0,T']\}$ for $T'=\left\lfloor log_2\left(\frac{T}{B}\right) \right\rfloor$. We begin at time $T>B$ so that there exists at least one model trained via Algorithm~\ref{alg:continualsampling}. At time $T=T'+b_0$ for some minimum batch size $b_0\in[1:B]$ consider the dataset $D^T_{(T-b_0+1, T)}$. This dataset represents the most recently arrived batch of data of size $b_0$, as shown in Figure ~\ref{fig:conthierarchy1}. For $b_0<<B$, the problem approaches continual release. On the other hand, if $ b_0 \approx B$, the problem approaches that of combining lower level models (e.g. trained using datasize $B$) with the current global model. The regularization term ensures that the new global model, $f^T$ remains close to the previous global model, $f_g$.

Suppose the updated model at time $T$ is denoted by $f^T$, then Equation~\ref{eq:regerm} defines a biased empirical risk minimization objective that can be used to obtain this updated global model. 
\begin{equation}\label{eq:regerm}
    f^T= \argmin_{w\in\mathcal{W}} \frac{1}{b_0}\sum_{i\in[1,b_0]} \ell(f(\mathbf{x}_i),y_i) + \lambda \norm{\mathbf{w} - \mathbf{w}_g}^2
\end{equation}
The model is released via a private empirical risk minimization algorithm, such as output perturbation based approaches outlined in Algorithm~\ref{alg:output}.\footnote{Note that the output perturbation approach  described in Algorithm~\ref{alg:privateERM} can be replaced by any private empirical risk minimization algorithm, including objective and gradient perturbation approaches, as long as the sensitivity and corresponding noise requirement has a factor of at least $O(\frac{1}{n})$. The last term in Theorem~\ref{thm:continual_utility} should also be updated appropriately. } 

%  \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.4\linewidth]{images/continualfig2.png}
%     \caption{Model Hierarchy in Continual Release}
%     \label{fig:conthierarchy2}
% \end{figure}

Now suppose another batch of data arrives, and we progress to an updated time $T^+$ for $T'+b_0<T^+<2T'$, as shown in Figure~\ref{fig:conthierarchy2}. At this point, we have access to the previous global model $f_g$, the most recent updated model $f^T$ and the new batch of data of size $b_0$,  denoted $D^{T^+}_{(T^+-b_0+1, T^+)}$. We proceed by updating $f^T$ to obtain the new up-to-date model $f^{T^+}$, again using a biased private empirical risk minimization algorithm in order to minimize the objective described by Equation~\ref{eq:regerm2}. 
\begin{equation}\label{eq:regerm2}
    f^{T^+}= \argmin_{w\in\mathcal{W}} \frac{1}{b_0}\sum_{i\in[1,b_0]} \ell(f(\mathbf{x}_i),y_i) + \lambda \norm{\mathbf{w} - \mathbf{w}_T}^2
\end{equation}


Continuing this process, we obtain a series of updated global models until $T^+=2T'$ when a new global model is obtained via Algorithm~\ref{alg:continualsampling}. Algorithm~\ref{alg:privateHTL} outlines the approach in full.

\begin{algorithm}[H]
\caption{Private Biased Regularized ERM (PB-ERM)}
\begin{algorithmic}[1]
  \scriptsize
  \STATE Input: Model to update $f_g$ parameterized by weights $\mathbf{w}_g$, new data $D^T_{(t-b_0+1, t)}$ , regularization constant $\lambda>0$, privacy parameter $\epsilon$, Lipschitz constant $L$.
    % \STATE{If relevant (e.g. SGD methods) initialize weights $\mathbf{w}_0=\mathbf{w}^S$}
    \STATE{$\mathbf{w}^T=\argmin_{w\in\mathcal{W}} \frac{1}{b_0}\sum_{i\in[1,b_0]} \ell(f(\mathbf{x}_i),y_i) + \lambda \norm{\mathbf{w} - \mathbf{w}_g}^2$}
    \RETURN{$\mathbf{w}^T+\nu$ where $\nu\sim Lap\left(\frac{2L}{\lambda b_0 \epsilon}\right)$}
\end{algorithmic}
  \label{alg:privateERM}
  \label{alg:pb-erm}
\end{algorithm}

\begin{algorithm}[H]
\caption{Private Continual Release via Hypothesis Transfer Learning}
\begin{algorithmic}[1]
  \scriptsize
  \STATE Input: Dataset $D=\{(\mathbf{x}_t, y_t) \}$ for $t\in \{B+1,...,T\}$, regularization constant $\lambda>0$, privacy parameter $\epsilon$, Lipschitz constant $L$, update batch size $b_0$. 
  \FOR{$t\in \{1, ..., T\}$} 
        \IF{$t!= 2^kB$ for $k\in [0, \lfloor log_2(\frac{t}{B})\rfloor]$ (not a global update step) \textbf{and}  $t\% b_0==0 $}
        \IF{$ t=\left\lfloor log_2\left( \frac{t}{B}\right)\right\rfloor + b_0$}
        \STATE{$T'=\left\lfloor log_2\left( \frac{t}{B}\right)\right\rfloor \hspace{2cm} \text{(First update since last global model)}$ }
        \ELSE
        \STATE{$T'=t-b_0 \hspace{2cm} \text{(Not first update since last global model)}$}
        \ENDIF
        \STATE{$f^T = PB-ERM( f^{T'},D^T_{(t-b_0+1, t)} )$.}
        \RETURN{ $f^T$}
        \ENDIF
  \ENDFOR
\end{algorithmic}
  \label{alg:privateHTL}
\end{algorithm}
\lauren{In Algorithm 5 we can do $T'=max()$ just thought an if-else was clearer for now}

\myparagraph{Privacy and Utility Guarantees}


\begin{theorem}[\citep{wu2017bolt, bassily2014private}]\label{thm:continualpriv}
Algorithm~\ref{alg:privateERM} satisfies $\epsilon$-differential privacy.
\end{theorem}

Algorithm~\ref{alg:privateHTL} performs $\epsilon$-differentially private updates via Algorithm~\ref{alg:privateERM} over disjoint paritions of a dataset $D^T$. Due to the parallel composition properties of Differential Privacy, Theorem~\ref{thm:continualpriv} demonstrates that Algorithm~\ref{alg:privateHTL} allows continual release of global models over the incoming dataset with only a constant increase in privacy loss in comparison to multi-resolution release using Algorithm~\ref{alg:continualsampling} alone. When used together, the total privacy loss of Algorithms~\ref{alg:continualsampling} and~\ref{alg:privateHTL} is then at most $2\epsilon$.

\begin{theorem}\label{thm:continualpriv}
Algorithm~\ref{alg:privateHTL} satisfies $\epsilon$-differential privacy.
\end{theorem}

Theorem~\ref{thm:continual_utility} bounds the excess empirical risk of the private models released via Algorithm~\ref{alg:privateHTL}. Denote the model output by Algorithm~\ref{alg:privateERM} by $\mathbf{w}_{priv}$ and the risk for the true minimizer $\mathbf{w}^*=\argmin_{\mathbf{w}}\mathbb{E}_{\mathcal{D}}[\ell(f(\mathbf{x}_i), y_i)]$. by $L(\mathbf{w}^*)$ . Denote the expected error of the model $f_g$ on the new data by $R_{g}$ and the weights before noise is added in Algorithm~\ref{alg:privateERM} by $\mathbf{w}^T_{np}$.
\lauren{Add in new window of data assume I.I.D (not I.I.D. over entire data stream) }
% \begin{theorem}\label{thm:continual_utility}
% Suppose the loss function used in Algorithm~\ref{alg:privateERM} is $L$-Lipschitz, $|\ell|_\infty\leq M$, $\Omega(\mathbf{w})=\lambda\norm{\mathbf{w}-\mathbf{w}_g}^2$, $H\leq\frac{b_0 \lambda}{2}$ and $\lambda=\sqrt{\frac{4L(1+\sqrt{4\eta})\sqrt{HR_{g}}}{\Omega(\mathbf{w}^T) b_0}}$ with $\mathbf{w}\in\mathbb{R}^d$, then we have that with probability at least $1-e^{-\eta}$: 
% \begin{equation}
%     \hat{L}_{priv}-L^* \leq \sqrt{\frac{2\eta R_{g}}{b_0}}+ \frac{ 1.5M \eta}{b_0}+(\Omega(\mathbf{w^*})-\Omega(\mathbf{w}^T_{np}))+\ln(\frac{d}{e^{-\eta}})\frac{2dL^2}{\lambda b_0 \epsilon}
% \end{equation}
% \end{theorem}
% \lauren{Where there is currently $(\Omega(\mathbf{w^*})-\Omega(\mathbf{w}^T_{np}))$ there could alternatively be $+2M$. See (\ref{eq:p2}) below. However, $2M$ could be large.  $(\Omega(\mathbf{w^*})-\Omega(\mathbf{w}^T_{np}))$ should be smaller than $2M$ if $\mathbf{w}^T_{np}$ and $w^*$ are close. How close they are should have a factor of $\frac{1}{b_0}$ in the strongly convex case but I haven't been able to work this out yet. Will continue to think about it. }

\begin{theorem}\label{thm:continual_utility}
Suppose the loss function used in Algorithm~\ref{alg:privateERM} is $L$-Lipschitz, $|\ell|_\infty\leq M$ and $\lambda\leq\frac{1}{\norm{\mathbf{w}^*-\mathbf{w}_g}^2 b_0}$ with $\mathbf{w}\in\mathbb{R}^d$, then with probability at least $1-e^{-\eta}$: 
\begin{equation}
    \hat{L}_D(\mathbf{w}_{priv})-L(\mathbf{w}^*) \leq \sqrt{\frac{2\eta R_{g}}{b_0}}+ \frac{ 1.5M \eta+1}{b_0}+\ln\left(\frac{d}{e^{-\eta}}\right)\frac{2dL^2}{\lambda b_0 \epsilon}
\end{equation}
\end{theorem}

\begin{proof}

Suppose $f^T$ is the output of Algorithm~\ref{alg:privateHTL} with corresponding weights $\mathbf{w}_T$. Note that $\mathbf{w}_T$ is the result of Algorithm~\ref{alg:privateERM}. Denote the non-private weights found by Algorithm~\ref{alg:privateERM}, before the addition of random noise, by $\mathbf{w}^T_{np}$. 

% Denote the true minimizer of the objective function before the addition of random noise by $w^*=\argmin_{\mathbf{w}}\mathbb{E}_{\mathcal{D}}[\ell(f(\mathbf{x}_i), y_i)]$. $\hat{L}(\mathbf{w})$ denotes the empirical risk. 

\[\hat{L}_D(\mathbf{w}_T)-L(\mathbf{w}^*) =\hat{L}_D(\mathbf{w}_T)-\hat{L}_D(\mathbf{w}^T_{np})+\hat{L}_D(\mathbf{w}^T_{np})-L(\mathbf{w}^*) \]


Due to Theorem 2 and Lemma 11~\citep{wu2017bolt}, using the Laplace Mechanism with noise scale $\nu\sim Lap(\frac{2L}{\lambda b_0\epsilon })$ to obtain $\mathbf{w}_{priv}$,
\[
    \hat{L}_D(\mathbf{w}_T)-\hat{L}_D(\mathbf{w}^T_{np}) \leq L\norm \nu \\
\]
So that with probability at least $1-e^{-\eta}$~\citep{wu2017bolt} ,
\begin{equation}\label{eq:q1}
    \hat{L}_D(\mathbf{w}_T)-\hat{L}_D(\mathbf{w}^T_{np}) \leq \ln\left(\frac{d}{e^{-\eta}}\right)\frac{2dL^2}{\lambda b_0 \epsilon}
\end{equation}
Note that $\hat{L}_D(\mathbf{w}^T_{np})-L(\mathbf{w}^*) = \hat{L}_D(\mathbf{w}^T_{np})-\hat{L}_D(\mathbf{w}^*)+\hat{L}_D(\mathbf{w}^*)-L(\mathbf{w}^*)$. Also, by definition, as $\mathbf{w}^T_{np}$ is the \textit{empirical minimizer}:
\[\hat{L}_D(\mathbf{w}^T_{np})+\lambda\norm{\mathbf{w}^T_{np}-\mathbf{w}_g}^2\leq \hat{L}_D(\mathbf{w}^*)+\lambda\norm{\mathbf{w}^*-\mathbf{w}_g}^2\]
\begin{equation}\label{eq:q2}
    \hat{L}_D(\mathbf{w}^T_{np})-\hat{L}_D(\mathbf{w}^*) \leq\lambda\norm{\mathbf{w}^*-\mathbf{w}_g}^2 - \lambda\norm{\mathbf{w}^T_{np}-\mathbf{w}_g}^2 \leq \lambda\norm{\mathbf{w}^*-\mathbf{w}_g}^2
\end{equation}
Recalling that $\lambda\leq\frac{1}{\Omega(w^*)b_0}$ we obtain:
\begin{equation}\label{eq:q3}
    \hat{L}_D(\mathbf{w}^T_{np})-\hat{L}_D(\mathbf{w}^*) \leq \frac{1}{b_0}
\end{equation}
Following~\cite{kuzborskij2013stability}, we then bound $\hat{L}(\mathbf{w}^*)-L(\mathbf{w}^*)$ using Bernstein's inequality to concentrate the empirical risk around its mean and noting that $L(\mathbf{w}^*)\leq R_g$:
\begin{align}
\hat{L}_D(\mathbf{w}^*)-L(\mathbf{w}^*) &\leq\sqrt{\frac{2\eta L(\mathbf{w}^*)}{b_0}}+ \frac{ 1.5M \eta}{b_0}\\
&\leq \sqrt{\frac{2\eta R_g}{b_0}}+ \frac{ 1.5M \eta}{b_0}\label{eq:q4}
\end{align}

Combining (\ref{eq:q1}), (\ref{eq:q3}) and (\ref{eq:q4}) we obtain the result.


\end{proof}
Theorem~\ref{thm:continual_utility} demonstrates that, as well as the expected relationship to $\epsilon$, both the size of the batch of data $b_0$ and the performance of the previous global model $R_{g}$ are important factors in reducing excess error. 


\subsection{Improved Continual Release}
We now propose extensions of Algorithm~\ref{alg:privateHTL} motivated by Theorem~\ref{thm:continual_utility}. We outline two methods to increase batch sizes, while maintaining continual monitoring of incoming data. Increasing batch size has two competing considerations. Firstly, increased batch size is directly motivated by the increased utility associated with larger batch datasizes in Theorem~\ref{thm:continual_utility}. However, if there is a significant change in underlying distribution at a given point in the incoming data stream, the continual release algorithm must quickly adapt by updating the model promptly. This motivates smaller batch sizes at some specific points in time. We also discuss selecting the optimal previous model to update, instead of automatically selecting the most recent global model. All extensions discussed increase the privacy loss in Theorem~\ref{thm:continualpriv} from $\epsilon$ to $2\epsilon$ due to the composition of Algorithm~\ref{alg:privateHTL} with a second $\epsilon$-differentially private algorithm.

\myparagraph{Combining Batches}

Suppose we denote the batches of size $b_0$ that arrived since $T=T'$ as $\{B_i:i\in[1,m]\}$. Now consider indices $i=2^k$ for $k\in[1, \lfloor log_2(m)\rfloor]$. At each of these indices, the total number of datapoints since $T'$ has doubled and we can apply the observations of Sections~\ref{sec:naive_multires} and~\ref{sec:sampling} to offer an alternative option for batches $B_h \in \{B_j:j=2^k\text{for} k\in[1, \lfloor log_2(m)\rfloor]\}$. For these batches, instead of using only the data in this batch in Algorithm~\ref{alg:privateHTL}, all datapoints that have arrived since $T'$ can be used. As before, this requires either fixed Laplace Noise $\nu \sim Lap\left( \frac{2L}{\lambda b_0 \epsilon} \right)$ or the addition of a sampling step to ensure a decreasing privacy loss of $\epsilon+\frac{\epsilon}{2}+ ... + \frac{\epsilon}{2^k} \leq 2\epsilon$ for each reused previous batch. 

\myparagraph{Lazy Batches}
\lauren{Will I delete this option as it may be 'too much' in terms of options?}
An alternative method is suggested by Online Learning algorithms in the non-private setting(refs), when updates are only made if an indicator measurement (e.g. accuracy of the previous global model over the new data) signals the need for an updated global model. Suppose we start with a batch of size $b_0$, we then evaluate if an update is needed immediately. If not, new incoming datapoints are added to the batch and the evaluation is updated. This process continues until a threshold is met, at which point Algorithm~\ref{alg:privateHTL} is used on this updated, larger batch of data. 


\myparagraph{Local Choice of Update Model}
Theorem~\ref{thm:continual_utility} demonstrates that the utility of any updated model is based on the 'goodness of fit' of the model being updated, $R_g$. This matches the intuition that we have biased the updated model to remain close to the model being updated. The optimal model to update for each new batch of data is the model that has the lowest error on that data (see Theorem~\ref{thm:continual_utility}). Therefore, the optimal model to update may not be the same for each new batch of data. The available models to update include:
\begin{itemize}
    \item The model $f_g$ alone, in other words the model at $a_1$ in Figure~\ref{fig:conthierarchy3}.
    \item A combination of the model $f_g$ and recent smaller models, for example in some scenarios a direct weighted combination of the form $\alpha_1 a_1+\alpha_2a_2$ for models at $a_1$ and $a_2$ in Figure~\ref{fig:conthierarchy3} with mixing weights $\alpha_1, \alpha_2 \in \mathbb{R}$.
    \item If applicable, the updated model obtained for the previous batch of data of size $b_0$.
\end{itemize}
\lauren{ left out option to just \textit{not} update one of these sources and copy one of them directly instead}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\linewidth]{images/hierarchy_continual2.png}
    \caption{Model Hierarchy in Continual Release}
    \label{fig:conthierarchy3}
\end{figure}

We select between these candidate source models using the Exponential Mechanism~\citep{mcsherry2007mechanism} where the quality score is the error of $f_g$ over the new batch of data. 

==> sections/multires.tex <==

\section{Multi-Resolution Release}

\rik{There is more to say about naive approaches. Suppose release a model every $t$, using standard composition, this gives $n$-DP. If we make use of the $1/n$ sensitivity, we get $\log n$-DP. 
}
\lauren{sure, I had these in the continual release section. I can reorder things to focus on continual release as the main point (see Trello list 'Overleaf Questions')}


Before outlining our solution to the problem stated in Section~\ref{sec:problem}, we will first discuss an $\epsilon$-differentially private \textit{multi-resolution release} method that is central to the private continual release approach described in Section~\ref{sec:continualrelease}. Multi-resolution release results in models solving the the empirical risk minimization problem described by (\ref{eq:erm}) for datasets of the form $D^T_{(t_1, t_2)}$ representing partitionings of $D^T$ into contiguous time intervals of size $s\in[B, 2B, ...., 2^kB]$ for   $k\in[1, \lfloor log_2(\frac{T}{B}) \rfloor]$. 


\myparagraph{Data Partitioning} Each datapoint indexed by $t\leq\lfloor\frac{T}{s}\rfloor s$ belongs to a single dataset of size $s$ for $s\in[B, 2B, ...., 2^kB]$. Note that there is  no overlap between datasets of the same size and that each of the datasets of size $2^jB$ is a subset of a single dataset of the form $D(2^kB, \cdot)$ for $j\leq k$, due to the contiguous manner of partitioning the incoming data stream. Each dataset of size $2^kB$ is the union of two datasets of size $2^{k-1}B$, as shown in Figure~\ref{fig:hierarchy}.
\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\linewidth]{images/cikm.png}
    \caption{Data partitioning hierarchy}
    \label{fig:hierarchy}
\end{figure}

Our \emph{multi-resolution release} problem therefore corresponds to releasing a hierarchy of private models for different lengths of time interval, where the total number of models released evolves dynamically as new data arrives. Multi-resolution release also results in the publication of a new global model over all datapoints that have arrived until time $T$ at exponentially increasing intervals of size $[B, 2B, .. 2^kB]$. 


\myparagraph{Shortcomings of Naive Approaches: }
We first address why a naive approach does not provide a satisfactory solution. The naive solution proceeds as follows: given a smallest time interval size of $B$, at time steps $t$ such that $t \pmod{B}= 0$, an $\epsilon$-differentially private model is released for the dataset $D^T_{(t-B, t)}$. If $t \pmod{2^kB} = 0$ for any $k\in [1, \lfloor log_2(\frac{T}{B}) \rfloor]$ then $\epsilon$-differentially private models are also released for the corresponding datasets of the form $D^T_{(t-2^kB, t)}$. This process continues as new data arrives. At time $T$, this approach results in a privacy guarantee of $\lfloor log_2(\frac{T}{B}) \rfloor \epsilon$ for any dataset of the form $D^T_{(t-B, t)}$, due to the composition properties of differential privacy. Therefore, as the datasize $T$ increases over time, no finite privacy budget can be satisfied by this algorithm without halting model release after some point in time. 

\subsection{Multi-Resolution Release Approach}\label{sec:naive_multires}
To address the shortcomings of the naive approach described above, we propose the following method that achieves multi-resolution release while incurring only a constant (finite) privacy loss of at most $\epsilon$.  This basic method, described in Algorithm~\ref{alg:multires}, forms the basis of all subsequent improved approaches proposed in this work. Algorithm~\ref{alg:output} describes a private stochastic gradient descent subroutine~\cite{chaudhuri2011differentially, bassily2014private, wu2017bolt}~\footnote{Note that in practice this subroutine can be substituted for any differentially private learning algorithm with sensitivity of $O(\frac{1}{n})$ given the corresponding sensitivity constant $C$ is set appropriately in Algorithm~\ref{alg:multires}. }

\begin{algorithm}
\caption{Private SGD via Output Perturbation (PSGD)~\cite{chaudhuri2011differentially, bassily2014private, wu2017bolt}}
\begin{algorithmic}[1]
  \scriptsize
  \STATE Input: $D=\{(\mathbf{x}_i, y_i) \}$, $n=|D|$, inverse learning rate $\gamma$, noise magnitude $\Delta_{\epsilon}$, training passes $k$.
  \STATE  $\mathbf{w} \leftarrow SGD(D)$ with $k$ passes and learning rate $ \frac{1}{\gamma i}$ for iteration $i$.
  \RETURN $\mathbf{w}+\nu$ where $\nu\sim Lap\left(\Delta_{\epsilon}\right)$.
\end{algorithmic}
  \label{alg:output}
\end{algorithm}
\abhirup{ Algo 1: Perhaps use a different notation for epoch other than $t$. Btw, the Algo 1 and 2 in Bolt-on paper sample noise from   exponential distribution.}

\lauren{ To me it seems Algorithm 2 of the bolt-on paper samples proportional to $ exp(-\frac{\epsilon |x|}{\Delta f}) $, the Laplace distribution with scale $b$ is given by $ exp(-\frac{|x|}{b})  )$? Appendix E also clarifies they are sampling Laplace noise. }

\begin{algorithm}
\caption{Private Multi-Resolution Release}
\begin{algorithmic}[1]
  \scriptsize
  \STATE Input: $D_T=\{(\mathbf{x}_t, y_t) \}$ for $t\in \{1,...,T\}$, $n_T=|D_T|$, block size $B$, sensitivity constant $C=\frac{4L}{\lambda B \epsilon}$ where $L$ is the Lipschitz constant.
   \FOR{$t\in \{1, ..., T\}$} 
        \FOR{$s \in \{B, ... 2^kB\}$ with $k\in [0, \lfloor log_2(\frac{T}{B}) \rfloor]$ }
            \IF{t \% s == 0} 
            \RETURN {  $\mathbf{w} \leftarrow PSGD(D=\{(\mathbf{x}_j, y_j) | j\in [t-2^kB+1, t]\}, \Delta_{\epsilon}=C)$ (Algorithm~\ref{alg:output})}  
            \ENDIF
        \ENDFOR
%   \STATE {Repeat lines 3-5 using $B\leftarrow 2^kB$ with $k\in [1, \lfloor log_2(\frac{T}{B}) \rfloor]$} and $D=\{(\mathbf{x}_j, y_j) | j\in [t-2^kB+1, t]\}$
   \ENDFOR
\end{algorithmic}
  \label{alg:multires}
\end{algorithm}
\abhirup{Algo 2: Perhaps we can make this cleaner?}
\lauren{Sure, is there a specific thing that seems off to you? Too much notation? Nested for loops?}

Algorithm~\ref{alg:multires} proceeds as follows: given a selected smallest time interval size of $B$, at time steps $t$ such that $t \pmod{B}= 0$, an $\frac{\epsilon}{2}$-differentially private model is released for the dataset $D^T_{(t-B, t)}$. Denote the scale of noise required to provide $\frac{\epsilon}{2}$-differential privacy for a dataset of size $B$ by the constant $C$. Following this, if $t \pmod{2^kB} = 0$ for any $k\in [1, \lfloor log_2(\frac{T}{B}) \rfloor]$ then differentially private models using noise of scale $C$ are also released for the appropriate datasets of the form $D^T_{(t-2^kB, t)}$. Given the use of a subroutine such as Algorithm~\ref{alg:output}, requiring noise of scale $\frac{1}{n}$ for a dataset of size $n$, the models released satisfy increasingly strong privacy guarantees of $\frac{\epsilon}{2\cdot2^k}$ as $k$ increases. The total privacy loss for any dataset of the form  $D^T_{(t-2B, t)}$ is then at most $\epsilon$ over any duration $T$, as demonstrated by Theorem~\ref{thm:basicprivacy}.

\begin{theorem} \label{thm:basicprivacy}
Algorithm~\ref{alg:multires} satisfies $\epsilon$-differential privacy.
\end{theorem}
\begin{proof}
% Consider data points  $(\mathbf{x}_t, y_t) \in D^T$. Denote the dataset of size $s\in[B, 2B, ...., 2^kB]$ that a point $(\mathbf{x}_t, y_t) \in D^T$ belongs to by $D^T(s, t)$ with $k\in[1, \lfloor log_2(\frac{T}{B}) \rfloor]$. As these datasets represent a partitioning of the dataset $D^T$ into blocks of size $s\in[B, 2B, ...., 2^kB]$. Each datapoint indexed by $t\leq\lfloor\frac{T}{s}\rfloor s$ belongs to a single dataset of the form $D^T(s, \cdot)$ for each value of $s$. Otherwise, this datapoint has not yet been used to train a model with datasize $s$.

% There is  no overlap between datasets of the same size and each of the datasets of size $2^jB$ is a subset of a single dataset of the form $D(2^kB, \cdot)$ for $j\leq k$, due to the contiguous manner of partitioning the incoming data stream. Each dataset of size $2^kB$ is the union of two datasets of size $2^{k-1}B$.

 Each model output in Algorithm~\ref{alg:multires} is released via the Laplace mechanism of Algorithm~\ref{alg:output}. Algorithm~\ref{alg:output} uses output perturbation to add Laplace Noise with scale $C$,  corresponding to the correct sensitivity to provide $\frac{\epsilon}{2}$-differential privacy for datasize $B$~\cite{chaudhuri2011differentially, bassily2014private, wu2017bolt}. Due the sensitivity of regularized empirical risk minimization of $\frac{2L}{\lambda n}$ for datasize $n$~\cite{wu2017bolt}, any model released using a datasize $2^kB$ for $k\in[0, \lfloor log_2(\frac{T}{B}) \rfloor]$ with fixed sensitivity $C$ satisfies $\frac{\epsilon}{2\cdot2^k}$-differential privacy. 
 
As noted in Section~\ref{sec:problem}, each datapoint belongs to a single model of each size $s\in[B, 2B, ...., 2^kB]$ and there is no overlap between datasets of the same size. Therefore, by the parallel composition properties of differential privacy~\cite{dwork2006calibrating}, the total privacy loss for any given datapoint (and its corresponding smallest dataset of size $B$) is  given by $\frac{\epsilon}{2}+\frac{\epsilon}{4}+... +\frac{\epsilon}{2\cdot2^{\lfloor log_2(\frac{T}{B}) \rfloor}}$ and we obtain the following geometric series: 
\begin{align*}
    \frac{\epsilon}{2}+\frac{\epsilon}{4}+... +\frac{\epsilon}{2\cdot2^{\lfloor log_2(\frac{T}{B}) \rfloor}} &= \epsilon\left(\frac{1}{2}+\frac{1}{4}+... +\frac{1}{2\cdot2^{\lfloor log_2(\frac{T}{B}) \rfloor}}\right) \\
    &\leq  \epsilon (1) \\
    &= \epsilon
\end{align*}


\end{proof}

Let us now consider the utility achieved by Algorithm~\ref{alg:multires}. Denote the output of a non-private stochastic gradient descent algorithm by $\mathbf{w}$, this corresponds to line 2 in Algorithm~\ref{alg:output}. Let $\mathbf{w}^*$ represent the non-private minimizer $\mathbf{w}^*=\argmin_{\mathbf{w}}\hat{L}_D(\mathbf{w})$. Denote the corresponding private released parameters by $\mathbf{w}_{priv}$. In other words, $\mathbf{w}_{priv}$ is the privatized set of parameters returned in line 3 of Algorithm~\ref{alg:output}. Theorem~\ref{thm:basicutility} describes the utility of Algorithm~\ref{alg:multires}.

\begin{theorem}[\textbf{\cite{wu2017bolt}}] . 
Consider 1-pass private stochastic gradient descent via Algorithm~\ref{alg:output} for $\beta$-smooth and $L$-Lipschitz loss function $\ell$. Suppose $sup_{\mathbf{w}\in\mathcal{W}}\|\ell'(\mathbf{w})\|\leq G$, $\mathcal{W}$ has diameter $R$ and $\mathcal{X}=\mathbb{R}^d$. Then, for a dataset of size $2^kB$ with $k\in[0, \lfloor log_2(\frac{T}{B})\rfloor]$
\begin{equation}
    \mathbb{E}[\hat{L}_D(\mathbf{w}_{priv})-\hat{L}_D(\mathbf{w}^*)]\leq \frac{((L+\beta R^2)+G^2)\log(2^kB)}{\lambda 2^kB}+\frac{4dG^2}{\epsilon \lambda B}
\end{equation}
\label{thm:basicutility}
\end{theorem}
% \lauren{Lauren: Isn't $G$ upper bounded by the lipschitz constant $L$? In the original paper for this result it seems not but I don't understand why, maybe a different norm?.}
Theorem~\ref{thm:basicutility} demonstrates that the cost of ensuring only constant privacy loss is that the excess privacy risk incurred remains the same as the datasize increases. Usually in private empirical risk minimization, the excess privacy risk incurred decreases as the datasize increases.  The first term in the bound provided in Theorem~\ref{thm:basicutility} is the upper bound for non-private excess risk $ \mathbb{E}[\hat{L}_D(\mathbf{w})-\hat{L}_D(\mathbf{w}^*)]$.  Therefore the excess risk due to differential privacy is bounded by $\frac{4dG^2}{\epsilon \lambda B}$ for each model produced by Algorithm~\ref{alg:multires}. 

 Section~\ref{sec:sampling} describes how the addition of a sampling procedure to Algorithm~\ref{alg:multires} results in a private continual release mechanism that achieves both a constant privacy loss overall and decreasing excess privacy risk as datasize increases.


==> sections/multiressampling.tex <==
\section{Improved Multi-Resolution Release with Sampling}\label{sec:sampling}

Previously, Algorithm~\ref{alg:multires} described a method allowing the multi-resolution release of private machine learning models, with only constant privacy loss over any period of time for any given data point. However, one implication of this method is that the same amount of noise is added to each model regardless of their underlying dataset size. Therefore, the utility of the released private models does not improve as underlying dataset size increases. To address this, we propose composing Algorithm~\ref{alg:multires} with a sampling procedure. This sampling procedure increases the level of sampling as underlying datasize increases. Due to amplification by subsampling~\cite{balle2018privacy}, Algorithm~\ref{alg:continualsampling} retains the crucial property of a constant overall privacy loss while also improving utility as datasize increases. 

\begin{algorithm}
\caption{Private Multi-Resolution Release with Sampling}
\begin{algorithmic}[1]
  \scriptsize
  \STATE Input: $D_T=\{(\mathbf{x}_t, y_t) \}$ for $t\in \{1,...,T\}$, $n_T=|D_T|$, block size $B$, sensitivity constant $C=\frac{4L}{\lambda B \epsilon}$ where $L$ is the Lipschitz constant.
   \FOR{$t\in \{1, ..., T\}$} 
        \FOR{$s \in \{B, ... 2^kB\}$ with $k\in [0, \lfloor log_2(\frac{T}{B}) \rfloor]$ }
            \IF{t \% s == 0} 
            \STATE{ $p_0 \rightarrow \frac{1}{2^k}$}
            \STATE {Let $D=\{(\mathbf{x}_j, y_j) | j\in [t-2^kB+1, t]\}$}
            \STATE {Obtain $D_{sample}$ by sampling without replacement from $D$ with probability $\frac{\exp{\big(\frac{\epsilon }{2}p_0\big)}-1}{\exp{\big(\frac{\epsilon}{2}\big)}-1}$ of including each data point.} 
            
            \RETURN { $\mathbf{w} \leftarrow PSGD(D=D_{sample}, \Delta_{\epsilon}=\frac{C}{2^k})$ (Algorithm~\ref{alg:output})}  
            \ENDIF
        \ENDFOR
        % \IF{t \% B == 0} 
        % \STATE {Let $D=\{(\mathbf{x}_j, y_j) | j\in [t-B+1, t]\}$}
        % \STATE {Obtain $D_{sample}$ by sampling without replacement from $D$ with probability $\frac{e^{\epsilon p_0/2}-1}{e^{\epsilon/2}-1}$} 
        % \STATE { Release model $\mathbf{w} \leftarrow PSGD(D=\{(\mathbf{x}_j, y_j) | j\in [t-B+1, t]\}, \Delta_{\epsilon}=C)$ (Algorithm~\ref{alg:output})}  
        % \ENDIF
%   \STATE {Repeat lines 3-5 using $B\leftarrow 2^kB$ with $k\in [1, \lfloor log_2(\frac{T}{B}) \rfloor]$ for $D=\{(\mathbf{x}_j, y_j) | j\in [t-2^kB+1, t]\}$. Substitute $p_0 \rightarrow \frac{p_0}{2^k}$ } and $\Delta_{\epsilon}=\frac{C}{2^k}$.
   \ENDFOR
\end{algorithmic}
  \label{alg:continualsampling}
\end{algorithm}

\begin{theorem} 
Algorithm~\ref{alg:continualsampling} satisfies $\epsilon$-differential privacy.
\end{theorem} 

\begin{proof}

For each of the datasets of size $2^kB$ for $k\in[0, \lfloor log_2(\frac{T}{B}) \rfloor]$ a model is released via the Laplace mechanism in Algorithm~\ref{alg:output}, adding Laplace Noise with sensitivity $\frac{4L}{\lambda 2^kB \epsilon}$. Denote Algorithm 1 by $A^1$. $A^1$ satisfies $\frac{\epsilon}{2}$-differential privacy for datasize $2^kB$~\cite{chaudhuri2011differentially, bassily2014private, wu2017bolt}.

% Denote Algorithm 1 by $A^1$. For all neighbouring datasets $D, D'$ and for all outputs $O\in Range(A^1)$,
% \begin{equation*}
%   \Pr[A^1(D) \in O] \leq e^{\frac{\epsilon}{2}} \cdot \Pr[A^1(D') \in O].
% \end{equation*}
Denote the composition of the sampling procedure outlined in Algorithm~\ref{alg:continualsampling} (line 7) with $A^1$ by $A^1_{samp}$. $A^1_{samp}$  satisfies $p_0\frac{\epsilon}{2}$-differential privacy ~\cite{li2012sampling, kellaris2013practical, beimel2014bounds, balle2018privacy}.As $p_0=\frac{1}{2^k}$ for $k\in[0, \lfloor log_2(\frac{T}{B}) \rfloor]$ and $A^1$ satisfies $\frac{\epsilon}{2}$-differential privacy, $A^1_{samp}$ satisfies $\frac{\epsilon}{2\cdot 2^k}$-differential privacy.

As outlined in the proof of Theorem~\ref{thm:basicprivacy}, due to the composition properties of differential privacy~\cite{dwork2006calibrating}, the total privacy loss for each block of size $B$ is then given by $\frac{\epsilon}{2}+\frac{\epsilon}{4}+... +\frac{\epsilon}{2\cdot2^{\lfloor log_2(\frac{T}{B}) \rfloor}}$. By the properties of geometric series we obtain: 
\begin{align*}
    \frac{\epsilon}{2}+\frac{\epsilon}{4}+... +\frac{\epsilon}{2\cdot2^{\lfloor log_2(\frac{T}{B}) \rfloor}} &= \epsilon\left(\frac{1}{2}+\frac{1}{4}+... +\frac{1}{2\cdot2^{\lfloor log_2(\frac{T}{B}) \rfloor}}\right) \\
    &\leq  \epsilon (1) \\
    &= \epsilon
\end{align*}

Therefore, Algorithm~\ref{alg:continualsampling} satisfies $\epsilon$-differential privacy.

\end{proof}

\begin{theorem}. 
Consider 1-pass private stochastic gradient descent via Algorithm~\ref{alg:continualsampling} for $\beta$-smooth and $L$-Lipschitz loss function $\ell$. Suppose $sup_{\mathbf{w}\in\mathcal{W}}\|\ell'(\mathbf{w})\|\leq G$, $\mathcal{W}$ has diameter $R$ and $\mathcal{X}=\mathbb{R}^d$. Then, for an input dataset of size $2^kB$ with $k\in[0, \lfloor log_2(\frac{T}{B})\rfloor]$ and subsample of size $n'$:
\begin{equation}
    \mathbb{E}[\hat{L}_D(\mathbf{w}_{priv})-\hat{L}_D(\mathbf{w}^*)]\leq \frac{((L+\beta R^2)+G^2)\log(n')}{\lambda n'}+\frac{4dG^2}{\epsilon \lambda 2^kB}
\end{equation}
\label{thm:samplingutility}
\end{theorem}
% Theorem: Utility (the privacy excess risk will now be $\frac{2dG^2}{\frac{\epsilon}{2}\lambda 2^kB}=\frac{4dG^2}{\epsilon\lambda 2^k B}$, question is what is the non-private first part after sampling... now high probability bound? )

\begin{proof}
Follows by Theorem~\ref{thm:basicutility}
\end{proof}

Note that with probability at least $1-\beta$, $n'\geq \left\lfloor \left(1-\sqrt{\frac{-2ln(\beta)}{B}}\right)B\right\rfloor$ and $\mathbb{E}[n']=B$.

Theorem~\ref{thm:samplingutility} describes the utility improvement achieved by Algorithm~\ref{alg:continualsampling}. The privacy risk decreases by a factor of $\frac{1}{2^k}$ to $\frac{4dG^2}{\epsilon \lambda 2^kB}$. The cost of this improvement is a corresponding decrease in datasize caused by sampling, as seen in the first term in the utility bound, the non-private excess risk $ \mathbb{E}[L_D(\mathbf{w})-L_D(\mathbf{w}^*)]$. The non-private excess risk depends on the datasize $n$ with a factor of $\frac{log(n)}{n}$. Sampling reduces the datasize from $2^kB$ to a datasize of at least $\left\lfloor \left(1-\sqrt{\frac{-2ln(\beta)}{B}}\right)B\right\rfloor$ with probability of at least $1-\beta$. 


==> sections/old_version_continual.tex <==
\section{Continual Release}

Algorithm~\ref{alg:continualsampling} provides a solution to the multi-scale release problem while simultaneously guaranteeing constant privacy loss over infinite timescales. A potential shortcoming of this method is that, while models representing smaller recent datasets are released at regular intervals, the most `global' model (covering all data up to time $T$) is only updated at exponentially growing time intervals of $B$, $2B$, $4B$, .. $2^kB$. After an appropriate burn-in period, this may be acceptable in an I.I.D. scenario. When the last global model represents a sufficient datasize, there will not be a large expected improvement in performance associated with adding small amounts of new data. Despite this, a potential issue arises in online and streaming scenarios where there is often no guarantee that non-I.I.D behaviour, such as concept drift or distribution shift, will not occur. A significant advantage of releasing multi-resolution models is that there is access to models trained using data that has recently arrived since the last global model. However, these models concern only a subset of the total dataset $D^T$ and natural next step is to ask if we can extend our algorithm to include the maintenance of an up-to-date global model at all time steps, in the style of \textit{continual release}. 

\subsubsection{Shortcomings of Naive Approaches}\label{subsec:naivecontinual} Naive approaches to the continual release of private empirical risk minimization algorithms suffer from significant degradation of privacy guarantees over time. For example, suppose we retrain a private empirical risk minimization algorithm each time a new datapoint arrives. Each model is $\epsilon$-differentially private. In this scenario the privacy of datapoints that arrived at the beginning of the data stream degrades to $T\epsilon$ at time $T$. If we instead use a sliding window of the $w$ most recent points for each value of $T\geq w$, then the privacy guarantee degrades to only $w\epsilon$ but at the cost of no longer performing true continual release over the entire existing dataset. Suppose instead that after a burn in period of $t_0$ datapoints we release trained models using constant Laplace noise, in the style of Algorithm~\ref{alg:continualsampling}. The privacy guarantee then degradades to $\epsilon(t_0ln(T)-t_0+1)$.



\subsection{Continual Release via Private Hypothesis Transfer Learning}

Our approach to continual release is based on Hypothesis Transfer Learning~\cite{kuzborskij2013stability}, a subset of techniques from Transfer Learning and Domain Adaptation. Transfer Learning focuses on improving the performance of machine learning models trained using a small dataset from a target distribution, aided by data from a larger related source domain. The goal is to transfer knowledge from the source domain to the target domain, thus aiding the learning process either in terms of accuracy or efficiency.  Hypothesis Transfer Learning focuses on scenarios in which only a hypothesis (e.g. a trained machine learning model) is known about the source domain, and there is no access to the source data itself when training a model for the target domain. This assumption is beneficial in private learning scenarios, as it avoids the pitfalls of composition discussed in~\ref{subsec:naivecontinual}. 

\subsubsection{Hypothesis Transfer Learning}
\lauren{We can move this description to the Background potentially} 

Consider a source dataset $D^S \sim \mathcal{X}^S\times\mathcal{Y}^S$, used to train a predictor $f^S : \mathcal{X}^S\rightarrow\mathcal{Y}^S$. Denote the target dataset by $D^T \sim \mathcal{X}^T\times\mathcal{Y}^T$ and the set of potential predictors by $f^T \in \mathcal{F}^T$ where $f^T:\mathcal{X}^T\rightarrow\mathcal{Y}^T$. 
A supervised learning algorithm $A$ using a dataset of size $m$ represents a map of the form $A: (\mathcal{X}^T\times\mathcal{Y}^T)^m\rightarrow f^T$. A Hypothesis Transfer Learning algorithm $A^{HTL}$ instread represents a mapping $A^{HTL}: (\mathcal{X}^T\times\mathcal{Y}^T)^m \times f^S \rightarrow f^T$. Generally, Hypothesis Transfer learning performs regularized empirical risk minimization over $D^T$, with a regularization term biasing $f^T$ to remain close to $f^S$. Suppose a model $f\in\mathcal{F^T}$ is parameterized by weights $\mathbf{w}\in\mathcal{W}^T$ and $f^S$ is parameterized by weights $\mathbf{w}^S\in\mathcal{W}^S$, then Equation~\ref{eq:htl} describes a hypothesis transfer learning objective.
\begin{equation}\label{eq:htl}
    f^T= \argmin_{w\in\mathcal{W}^T} \frac{1}{m}\sum_{i\in[1,m]} \ell(f(\mathbf{x}_i),y_i) + \lambda \norm{\mathbf{w} - \mathbf{w}^S}^2
\end{equation}

The source hypothesis can also be composed of multiple hypotheses $f^S = \sum_i \beta_i f^{S_i}$ from multiple potential source datasets $D^{S_i}\sim \mathcal{X}^S\times\mathcal{Y}^S$.  

\subsubsection{Adapting Hypothesis Transfer Learning for Private Continual Release} 
We begin at time $T>B$ so that there exists at least one model trained via Algorithm~\ref{alg:continualsampling}. Let $f^S$ be either the last `global' model trained (model $a_1$ in Figure~\ref{fig:hierarchy}) or a weighted sum of this global model with other smaller models (model $a_2$ in Figure~\ref{fig:hierarchy}) released via Algorithm~\ref{alg:continualsampling} since the last global model was trained. Each of these models satisfies differential privacy. Therefore due to immunity to post-processing, their use does not leak further information about the data previously used to train them.

Suppose the last global model was trained using datasize $g$. From time $T$ until a new global model is trained at time $2g$, we consider the new incoming data in batches of minimum size $b_0\in[1:B]$. For $b_0<<B$, the problem approaches continual release. If  $ b_0 \approx B$, the problem approaches that of combining lower level models with the current global model. 
\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{images/hierarchy_continual2.png}
    \caption{Model Hierarchy in Continual Release}
    \label{fig:conthierarchy}
\end{figure}

Our goal is to fine-tune $f^S$ using each newly arrived batch of data of size $b_0$ in order to maintain a continually updated model $f^T$ that includes information on all data arrived until time $T$.

\subsubsection{Local Choice of Source Hypothesis}\label{subsubsec:source}
The optimal source hypothesis for each new batch of data is the model hypothesis that has the lowest error on that data (see Theorem~\ref{thm:continual_utility}). Therefore, the optimal source model may not be the same for each new batch of data. The available source hypotheses include:
\begin{itemize}
    \item The previous global model alone, model $a_1$ in Figure~\ref{fig:conthierarchy}.
    \item A weighted combination of the global model and recent smaller models, $\beta_1 a_1+\beta_2a_2$ for models $a_1$ and $a_2$ in Figure~\ref{fig:conthierarchy} with mixing weights $\beta_1, \beta_2 \in \mathbb{R}$.
    \item The updated model obtained for the previous batch of data of size $b_0$. If $T>g+b_0$ then this is the model $f^{T'}$ for $T'=T-b_0$.
\end{itemize}
\lauren{ left out option to just \textit{not} update one of these sources and copy one of them directly instead}

We select between these candidate source models using the Exponential Mechanism~\cite{mcsherry2007mechanism} where the quality score is the error of $f^S$ over the new batch of data of size $b_0$, denoted by $D'$. 

\subsubsection{Fine-Tuning on the Target Domain}
Hypothesis Transfer Learning is then performed on the the new batch of data $D'$, using the selected source model $f^S$. This is performed using a private regularized empirical risk minimization algorithm, such as Algorithm~\ref{alg:privateERM} initialized at $f^S$, for the objective described by (\ref{eq:htl}). Note that the objective remains $\lambda$-strongly convex and therefore the privacy noise required in Algorithm~\ref{alg:output} is unchanged in this context.\footnote{Note that while an output perturbation approach is described in Algorithm~\ref{alg:privateERM}, this can be replaced by any private empirical risk minimization algorithm including objective and gradient perturbation approaches, with the last term in Theorem~\ref{thm:continual_utility} updated appropriately. }
\begin{algorithm}
\caption{Private Regularized ERM (HTL-PERM}
\begin{algorithmic}[1]
  \scriptsize
  \STATE Input: Source model $f^S$ parameterized by weights $\mathbf{w}^S$, new data $D'=\{(\mathbf{x}_t, y_t) \}$ for $t\in \{1,...,b_0\}$, regularization constant $\lambda>0$, privacy parameter $\epsilon$, Lipschitz constant $L$.
    % \STATE{If relevant (e.g. SGD methods) initialize weights $\mathbf{w}_0=\mathbf{w}^S$}
    \STATE{$\mathbf{w}^T=\argmin_{w\in\mathcal{W}^T} \frac{1}{m}\sum_{i\in[1,b_0]} \ell(f(\mathbf{x}_i),y_i) + \lambda \norm{\mathbf{w} - \mathbf{w}^S}^2$}
    \RETURN{$\mathbf{w}^T+\nu$ where $\nu\sim Lap\left(\frac{2L}{\lambda b_0 \epsilon}\right)$}
\end{algorithmic}
  \label{alg:privateERM}
\end{algorithm}

\begin{algorithm}
\caption{Private Continual Release via Hypothesis Transfer Learning}
\begin{algorithmic}[1]
  \scriptsize
  \STATE Input: Dataset $D=\{(\mathbf{x}_t, y_t) \}$ for $t\in \{B+1,...,T\}$, regularization constant $\lambda>0$, privacy parameter $\epsilon$, Lipschitz constant $L$. 
  \FOR{$t\in \{1, ..., T\}$} 
        \IF{$t!= 2^kB$ for $k\in [0, log_2(\frac{t}{B})]$ (not a global update step) \textbf{and}  $t\% b_0==0 $}
        \STATE{$f^T = HTL-PERM(D', f^S)$ where $D'=\{(\mathbf{x}_t, y_t) \}$ for $t\in \{t-b_0+1,...,t\}$ with $f^S$ selected according to~\ref{subsubsec:source}.}
        \RETURN{ $f^T$}
        \ENDIF
  \ENDFOR
\end{algorithmic}
  \label{alg:privateHTL}
\end{algorithm}
\subsubsection{Privacy and Utility Guarantees}
Through direct application of the composition properties of Differential Privacy, combined with the fact that the continual release models are trained over disjoint datasets, Theorem~\ref{thm:continualpriv} demonstrates that Algorithm~\ref{alg:privateHTL} provides the continual release of global models over the incoming dataset, with only a constant increase in privacy loss in comparison to multi-resolution release using Algorithm~\ref{alg:continualsampling} alone. 

\begin{theorem}\label{thm:continualpriv}
Algorithm~\ref{alg:privateHTL} satisfies $2\epsilon$-differential privacy.
\end{theorem}
Extending previous work on Hypothesis Transfer Learning~\cite{kuzborskij2018theory}, we obtain a bound on the excess empirical error of the private hypothesis transfer learning models. Denote the empirical risk of the model output by Algorithm~\ref{alg:privateERM} by $\hat{L}_{priv}$ and empirical risk for the true minimizer by $L^*$. Denote the expected error of the source hypothesis on the target data by $R^{src}$
\begin{theorem}\label{thm:continual_utility}
Suppose the loss function used in Algorithm~\ref{alg:privateERM} is $L$-Lipschitz, $|\ell|_\infty\leq M$, $\omega=\lambda\norm{\mathbf{w}^T-\mathbf{w}^S}^2$, $H\leq\frac{b_0 \lambda}{2}$ and $\lambda=\sqrt{\frac{4L(1+\sqrt{4\eta})\sqrt{HR^{src}}}{\omega b_0}}$, then we have that with probability at least $1-e^{-\eta}$: 
\begin{equation}
    |\hat{L}_{priv}-L^*| \leq \sqrt{\frac{2\eta R^{src}}{b_0}}+ \frac{1.5 M \eta}{b_0}-\ln(1-e^{-\eta})\frac{2L^2}{\lambda b_0 \epsilon}
\end{equation}\end{theorem}
Theorem~\ref{thm:continual_utility} demonstrates that, as well as the expected relationship to $\epsilon$, both the size of the batch of data $b_0$ and the performance of the source model $R^{src}$ are important factors in reducing excess error. Note that if the source is a good fit and $R^{src}$ is small, the dominant terms have a factor of $O(\frac{1}{b_0})$ .
\subsection{Improved Private Hypothesis Transfer Learning}
We now present two methods to increase batch sizes, while maintaining continual monitoring of incoming data. Increasing batch size has two competing considerations. Firstly, increased batch size is directly motivated by the increased utility associated with larger target domain datasizes in Theorem~\ref{thm:continual_utility}. However, if there is a significant change in underlying distribution at a given point in the incoming data stream, the continual release algorithm must quickly adapt by updating the model promptly. This motivates smaller batch sizes at some specific points in time.  

\subsubsection{Combining Batches}

Suppose we label the batches of size $b_0$ since the last global model update as $B_i$ for $i\in[1,w]$. Now consider indices $h=2^k$ for $k\in[1, \lfloor log_2(w)\rfloor]$. At each of these indices, the total number of datapoints since the last global model update has doubled and we can apply the observations of Sections~\ref{sec:naive_multires} and~\ref{sec:sampling} to offer an alternative HTL option for batches $B_h$. For these batches, instead of using only the data in this batch in Algorithm~\ref{alg:privateHTL}, all datapoints that have arrived since the last global model update can be used. As before, this requires either fixed Laplace Noise $\nu \sim Lap\left( \frac{2L}{\lambda b_0 \epsilon}\right)$ or the addition of a sampling step to ensure a decreasing privacy loss of $\epsilon+\frac{\epsilon}{2}+ ... + \frac{\epsilon}{2^k} \leq 2\epsilon$ for each reused previous batch. 

\subsubsection{Lazy Batches}
\lauren{Will I delete this option as it may be 'too much' in terms of options?}
An alternative method is suggested by Online Learning algorithms in the non-private setting(refs), when updates are only made if an indicator measurement (e.g. accuracy of the previous global model over the new data) signals the need for an updated global model. In our setting, we start with a batch of size $b_0$, we evaluate if an update is needed immediately, if not new incoming datapoints are added to the batch and the evaluation is updated. This process continues until a threshold is met, at which point Algorithm~\ref{alg:privateHTL} is used on this updated batch of data. 


==> sections/slidingwindow.tex <==
\section{Sliding Window Release}

Algorithm~\ref{alg:privateHTL} describes private empirical risk minimization in a continual release scenario, over a potentially infinite timescale with only constant privacy loss. We now consider another style of continual release. Specifically, consider settings where only the last window of data of size $w$ is relevant at any time $T$. In this scenario, access to an updated model over a continually evolving sliding window of recent data would be preferable to either a global continual release model or models over fixed windows of data.  Let $D^T_{w}=\{(\mathbf{x}_t, y_t): t\in[T-w+1, T]\}$, our goal is to release a solution to the regularized empirical risk minimization problem defined in (\ref{eq:erm}) as $T$ evolves over time, for all $T\geq w$. 

\myparagraph{Naive Methods}
Consider a naive sliding window algorithm that releases an $\epsilon$-differentially private model for each new window of size $w$ for each $t\in[w:T]$, in other words for all datasets of the form $D^t_{(t-w+1, t)}$. By composition, this results in a privacy guarantee of $w\epsilon$. As $w$ may be large, this could indicate an unacceptable level of privacy loss.

\subsection{Sliding Window Algorithm}
Consider a window of size $w$, denoted by $D^T_{(t-w+1, t)}=\{(\mathbf{x}_i, y_i):i\in[T-w+1, T]\}$. Suppose this window can then be split into blocks of the form $w=\sum_{j\in[0,\lfloor log_2(w/w_0)\rfloor]}^{h} 2^{j}w_0$, as shown in Figure~\ref{fig:sliding1}, $w_0$ represents the minimum update size. 

\begin{figure}[h]
    \centering
    \begin{minipage}{.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/sliding1.png}
    \caption{Sliding window size $w$, $w_0=1$.}
    \label{fig:sliding1}
    \end{minipage}%
    \begin{minipage}{0.5\textwidth}
        \centering
    \includegraphics[width=\linewidth]{images/sliding2.png}
    \caption{Sliding window size $w$, $w_0=1$.}
    \label{fig:sliding2}
    \end{minipage}
\end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.4\linewidth]{images/sliding1.png}
%     \caption{A sliding window of size $w$, with $w_0=1$.}
%     \label{fig:sliding1}
% \end{figure}

Algorithm~\ref{alg:slidingwindow} proceeds as follows. For the largest block of data with size $2^{\lfloor log_2(w/w_0)\rfloor}w_0$, an $\epsilon$-differentially private model is released, trained using a private empirical risk minimization technique such as Algorithm~\ref{alg:output}. Denote this model by $f^0$, we then employ the fine-tuning method previously used in Algorithm~\ref{alg:privateHTL} to sequentially include the datapoints in smaller blocks, until a global model for the window is obtained.  This is shown in Figure~\ref{fig:sliding2}.
Now consider timestep $T+w_0$, when the sliding window has moved by one block. In this scenario, we simply update the model $f^2$ in Figure~\ref{fig:sliding2} using the new block of data, as shown in Figure~\ref{fig:sliding3}. 

\begin{figure}[h]
    \centering
    \begin{minipage}{.5\textwidth}
        \centering
   \includegraphics[width=\linewidth]{images/sliding3.png}
    \caption{Sliding window size $w$, $w_0=1$.}
    \label{fig:sliding3}
    \end{minipage}%
    \begin{minipage}{0.5\textwidth}
        \centering
    \includegraphics[width=\linewidth]{images/sliding4.png}
    \caption{Sliding window size $w$, $w_0=1$.}
    \label{fig:sliding4}
    \end{minipage}
\end{figure}

At the next time step $T+2w_0$ shown in Figure~\ref{fig:sliding4} , we adjust the location of blocks of size $2^1$ and $2^0$ and update $f^1$ appropriately. This process continues until the window passes the existing largest block with model $f^0-$ trained using datasize $2^{\lfloor log_2(w/w_0)\rfloor}w_0$. At this point, the partitioning and model training process begins from scratch, as first shown in Figure~\ref{fig:sliding2}.

\lauren{I assume we can mode 6 and 7 to an appendix or massively simplify how much detail the algorithm description gives.}
\begin{algorithm}[H]
\caption{Initialize Window ($WindowInit$)}
\begin{algorithmic}[1]
  \scriptsize
    \STATE Input: Data Window $D^w=\{(\mathbf{x}_i, y_i) : i \in [1, w]\}$ , regularization constant $\lambda>0$, privacy parameter $\epsilon$, Lipschitz constant $L$, window size $w$, minimum update size $w_0$.
    \STATE{$T'=2^{\lfloor log_2(w/w_0)\rfloor}$} \algorithmiccomment{Size of largest power of 2 block}
    \STATE{$D^{T'}=D^w_(w-T'w_0+1,w)$}
    \STATE{$\mathbf{w}^{T'}=\argmin_{w\in\mathcal{W}} \frac{1}{b_0}\sum_{i\in[1,b_0]} \ell(f(\mathbf{x}_i),y_i) + \lambda \norm{\mathbf{w} - \mathbf{w}_g}^2$}
    \STATE{$f^{T'}$ is parameterized by $\mathbf{w}^T+\nu$ where $\nu\sim Lap\left(\frac{4L}{\lambda w_0
\epsilon}\right)$}
    \FOR{$j\in reverse([1,\lfloor log_2(w/w_0)\rfloor-1])$}
    \STATE{$D^{new}=D^w_{(2^{j-1}w_0+1, 2^jw_0)}$}
    \IF{$j=\lfloor log_2(w/w_0)\rfloor-1$}
    \STATE{$f^j \leftarrow PB-ERM(f_g=f^{T'}, D^{new}, \text{noise scale}= \frac{6L}{\lambda w_0
\epsilon})$}
    \ELSE{ }
    \STATE{$f^j \leftarrow PB-ERM(f_g=f^{j+1}, D^{new}, \text{noise scale}= \frac{6L}{\lambda w_0
\epsilon})$}
    \ENDIF
    \ENDFOR
    \RETURN{ $[f^{T'},  \{f^j:j\in reverse([1,\lfloor log_2(w/w_0)\rfloor-1])\}$}
\end{algorithmic}
  \label{alg:wndowinit}
\end{algorithm}

\begin{algorithm}[H]
\caption{Model Update ($ModelUpdate$)}
\begin{algorithmic}[1]
  \scriptsize
  \STATE{Input: Dataset $D^T$ , regularization constant $\lambda>0$, privacy parameter $\epsilon$, Lipschitz constant $L$, window size $w$, minimum update size $w_0$.}
  \STATE{Update partitioning of $D^w$ into batches of size $[2^0w_0, ..., 2^{\lfloor log_2(w/w_0)\rfloor}-1]$.}
  \STATE{Suppose subsets $D^w_{(2^{k-1}w_0, 2^kw_0)}$ for $k\in[0, K]$ are changed in comparison to step $t-1$}
   \FOR{$j\in reverse([1,K])$}
    \STATE{$f^j \leftarrow PB-ERM(f_g=f^{j+1}, D^w_{(2^{j-1}w_0+1, 2^jw_0)}, \text{noise scale}= \frac{6L}{\lambda w_0
\epsilon})$}
    \ENDFOR
\RETURN{Updated values of $[f^{T'},  \{f^j:j\in reverse([1,\lfloor log_2(w/w_0)\rfloor-1])\}$}\end{algorithmic}
  \label{alg:modelupdate}
\end{algorithm}




\begin{algorithm}[H]
\caption{Private Sliding Window ERM ($PSW-ERM$)}
\begin{algorithmic}[1]
  \scriptsize
  \STATE Input: Dataset $D^T$ , regularization constant $\lambda>0$, privacy parameter $\epsilon$, Lipschitz constant $L$, window size $w$, minimum update size $w_0$.
    \STATE{$T'=2^{\lfloor log_2(w/w_0)\rfloor}$} \algorithmiccomment{Size of largest power of 2 block}
    \STATE{$lastInit=t$} \algorithmiccomment{Last time window was intialized to match Figure~\ref{fig:sliding1}}
    \STATE{$maxGap=w-T'w_0$} \algorithmiccomment{Steps before we reach the largest block}
      \FOR{$t\in[w,T]$}
    \IF{$t==w$}
    \STATE{$[f^{T'w_0}, ... , f^w]= WindowInit(D^T_{(t-w+1, t)})$ }
    \ELSIF{$t=lastInit+kw_0$ for $k=\in[1, \lfloor w/w_0\rfloor]$ AND $t<lastInit+maxGap+1$}
    \STATE{$[f^{T'w_0}, ... , f^w]= ModelUpdate(D^T_{(t-w+1, t)}))$ }
    \ELSIF{$t=lastInit + maxGap+1$}
    \STATE{$[f^{T'w_0}, ... , f^w]= WindowInit(D^T_{(t-w+1, t)})))$}
    \STATE{$lastInit=t$}
    \ENDIF
    \RETURN{$f^w$}
   \ENDFOR
\end{algorithmic}
  \label{alg:slidingwindow}
\end{algorithm}

\myparagraph{Privacy and Utility Guarantees}
Algorithm~\ref{alg:slidingwindow} allows the release of continually updated ERM models over a sliding window of data, with only constant privacy loss. 
\begin{theorem}
Algorithm~\ref{alg:slidingwindow} satisfies $\epsilon$-differential privacy.
\end{theorem}




\begin{proof}
Consider the timestep directly following a call of Algorithm~\ref{alg:wndowinit}, when the window of data is in the format shown in Figure~\ref{fig:sliding1}. Denote the dataset representing the window of size $w$ at this timestep by $D^w=\{\mathbf{x}_i, y_i : i\in[1,w]\}$. Let $w=\sum_{j=1}^J 2^jw_0$. We consider a single pass of the sliding window algorithm over $D^w$, before the next call of Algorithm~\ref{alg:wndowinit} which will reset the window. Note that this extends the data used by the algorithm from just $D^w$ originally, to $D^{w^+}=\{\mathbf{x}_i, y_i : i\in[1,w+2^Jw_0-1]\}$ before the window is refreshed.

We consider the following three disjoints datasets for the $k^{th}$ pass of the sliding window algorithm. These datasets represent a partitioning of $D^{w^+}$ into the data before the largest model, the data contained in the largest model, and the data that arrives after the largest model during this pass of the sliding window algorithm:
\begin{itemize}
    \item $D_k^L=\{\mathbf{x}_i, y_i : i\in[1,(2^J-1)w_0]\}$
    \item $D_k^R=\{\mathbf{x}_i, y_i : i\in[(2^J-1)w_0+1,w]\}$
    \item $D_k^{R+}=\{\mathbf{x}_i, y_i : i\in[w+1, w+2^Jw_0-1]\}$
\end{itemize}

Note that at at the $(k-1)^{th}$ pass of the sliding window algorithm $D_{k-1}^R=D_j^L$ and $D_{k-1}^{R+}=D_k^R$. If we also consider the $(k+1)^{th}$ pass of the algorithm, then $D_{k+1}^L=D_k^R=D_{k-1}^{R+}$ and $D_{k+1}^{R}=D_k^{R+}$. Therefore over all passes of the sliding window algorithm, each of the disjoint datasets represented above will be used three times, as effectively $D_{k+1}^L, D_k^R$ and $D_{k+1}^{R+}$ for some value of $k$.

Due to this observation, the differential privacy guarantee for Algorithm~\ref{alg:slidingwindow} follows immediately from the fact that Algorithm~\ref{alg:slidingwindow} satisfies $\frac{\epsilon}{3}$-differential privacy over a single pass $j$ for each of these datasets, as demonstrated below.

It follows immediately from the privacy guarantee of Algorithm~\ref{alg:output}, outlined in the proof of Theorem~\ref{thm:basicprivacy}, that Algorithm~\ref{alg:slidingwindow} satisfies $\frac{\epsilon}{3}$-differential privacy for dataset $D^R$. Only a single private empirical risk minimization algorithm with appropriately added noise is released using dataset $D^R$ before a window refresh. 

The privacy guarantee for Algorithm~\ref{alg:slidingwindow} over $D^{R+}$ and $D^L$ are identical as both call Algorithm~\ref{alg:privateERM} for models of sizes $2^0, .. 2^{J-1}$ using Laplace noise with scale $\frac{6L}{\epsilon w_0 \lambda}$ in Algorithm~\ref{alg:privateERM}, therefore satisfying $\frac{\epsilon}{3}$-differential privacy over one pass of the sliding window algorithm due to~\cite{bassily2014private} and the argument previously used in Theorem~\ref{thm:basicprivacy}. 

% Denote the dataset representing any window of size $w$ by $D^w=\{\mathbf{x}_i, y_i : i\in[1,w]\}$. 
% Let $w=\sum_{j=1}^J 2^jw_0$ and consider the privacy loss of the two disjoint datasets $D^L=\{\mathbf{x}_i, y_i : i\in[1,\sum_{j\in[0, J-1]} 2^jw_0]\}$ and $D^R=\{\mathbf{x}_i, y_i : i\in[w-2^Jw_0+1,w]\}$ at a time step directly following a window initialization e.g. when the window is of the form show in Figure~\ref{fig:sliding1}. These datasets represent all data points not included in the largest trained model, and all data points included in the largest trained model respectively at that time step. The largest trained model is denoted by $f^0$ in Figures~\ref{fig:sliding2}-\ref{fig:sliding4}. 

% We will demonstrate that the privacy loss of Algorithm~\ref{alg:slidingwindow} on both of these datasets is at most $\frac{\epsilon}{3}$ over one full pass of the sliding window, until the point when the window is refreshed. In other words, until the $WindowInit$ method outlined in Algorithm~\ref{alg:wndowinit} is called. This proves our claim when combined with the observation that these datasets will have no overlap when the window is refreshed as $w=\sum_{i\in[0, J]} 2^jw_0= \sum_{i\in[0, J-1]} 2^jw_0 + 2^Jw_0 = 2^Jw_0 - 1 + 2^Jw_0$ and are effectively used three times by the Algorithm. 

% A key observation is that $D^R$ in this particular window of data was previously


% Each of these datasets will be used once as the left hand side dataset, once as the right hand side dataset (the largest model) by Algorithm~\ref{alg:slidingwindow} and once as the 'far-right dataset'. The far right datasets denoted  $D^{R+}=\{\mathbf{x}_i, y_i : i\in[w, w+2^Jw_0-1]\}$, represents the data that is accumulated to the right hand side of $D^R$ before a window refresh (and is effectively $D^R$ in the next pass of the algorithm). The privacy guarantee for Algorithm~\ref{alg:slidingwindow} over $D^{R+}$ and $D^L$ are identical as both call Algorithm~\ref{alg:privateERM} for models of sizes $2^0, .. 2^{J-1}$ using Laplace noise with scale $\frac{6L}{\epsilon w_0 \lambda}$ in Algorithm~\ref{alg:privateERM}, therefore satisfying $\frac{\epsilon}{3}$-differential privacy over one pass of the sliding window algorithm due to~\cite{bassily2014private} and the argument previously used in Theorem~\ref{thm:basicprivacy}. 

% It follows immediately from the privacy guarantee of Algorithm~\ref{alg:output}, outlined in the proof of Theorem~\ref{thm:basicprivacy}, that Algorithm~\ref{alg:slidingwindow} satisfies $\frac{\epsilon}{3}$-differential privacy for dataset $D^R$. Only a single private empirical risk minimization algorithm with appropriately added noise is released using dataset $D^R$ before a window refresh. 

% Therefore as each of the three uses of the datasets $D^L$ and $D^R$ is $\frac{\epsilon}{3}$-differentially private, Algorithm~\ref{alg:slidingwindow} satisfies $\epsilon$-differentially private via sequential composition.


\end{proof}
% Denote the model that is updated to provide the final window model $f^w$ by $f^{-1}$, parameterized by weights $\mathbf{w}_{-1}$.  For example,  $f^{-1}$ corresponds to model $f^2$ in Figure~\ref{fig:sliding2} or model $f^5$ in Figure~\ref{fig:sliding4}. 


Denote the private released model for the window by $f^w$, parameterized by weights $\mathbf{w}$. The model $\mathbf{w}$ before the addition of Laplace Noise is instead denoted by $\mathbf{w}_{np}$. As before, the true minimizer is denoted by $\mathbf{w}^*=\argmin_{\mathbf{w}}\mathbb{E}_{\mathcal{D}}[\ell(f(\mathbf{x}_i), y_i)]$. 
\begin{theorem}\label{thm:sliding_utility }
Suppose the loss function used in Algorithm~\ref{alg:slidingwindow} is $L$-Lipschitz, $|\ell|_\infty\leq M$, $\Omega(\mathbf{w})=\norm{\mathbf{w}-\mathbf{w}_{-1}}^2$, and $\lambda\leq\frac{1}{\Omega(\mathbf{w}^*) w_0}$ with $\mathbf{w}\in\mathbb{R}^d$, then with probability at least $1-e^{-\eta}$: 
\begin{equation}
    \hat{L}_D(\mathbf{w})-L(\mathbf{w}^*) \leq \sqrt{\frac{2\eta L(\mathbf{w}^*)}{w_0}}+ \frac{ 1.5M \eta+1}{w_0}+\ln(\frac{d}{e^{-\eta}})\frac{6dL^2}{\lambda w_0 \epsilon}
\end{equation}
\end{theorem}

\begin{proof}
This result is obtained via similar reasoning to Theorem~\ref{thm:continual_utility}, recognizing that the final model output for a window is essentially the result of private regularized empirical risk minimization using the regularizer described in Equation~\ref{eq:regerm}. In the sliding window scenario, the weights $w_g$ used in the regularizer correspond to the most recently updated larger block of data within the window (e.g. model $f^2$ in Figure~\ref{fig:sliding2} or model $f^5$ in Figure~\ref{fig:sliding4}). 

Suppose $f^w$ is the output of Algorithm~\ref{alg:slidingwindow} for a given window of data, with corresponding weights $\mathbf{w}$. Note that $\mathbf{w}$ is the result of Algorithm~\ref{alg:privateERM} using noise of scale $\frac{6L}{\lambda w_0 \epsilon}$. Denote the non-private weights found by Algorithm~\ref{alg:privateERM}, before the addition of random noise, by $\mathbf{w}_{np}$. Denote the true minimizer of the objective function before the addition of random noise by $w^*$, with corresponding risk $L(\mathbf{w}^*)$. $\hat{L}_D(\mathbf{w})$ denotes the empirical risk. 

\[\hat{L}_D(\mathbf{w})-L(\mathbf{w}^*)  =\hat{L}_D(\mathbf{w})-\hat{L}_D(\mathbf{w}_{np})+\hat{L}_D(\mathbf{w}_{np})-L(\mathbf{w}^*)  \]


Due to Theorem 2 and Lemma 11~\citep{wu2017bolt}, using the Laplace Mechanism with noise scale $\nu\sim Lap(\frac{6L}{\lambda w_0\epsilon })$ to obtain $\mathbf{w}$,
\[
    \hat{L}_D(\mathbf{w})-\hat{L}_D(\mathbf{w}_{np}) \leq L\norm \nu \\
\]
So that with probability at least $1-e^{-\eta}$~\citep{wu2017bolt} ,
\begin{equation}\label{eq:p1}
    \hat{L}_D(\mathbf{w})-\hat{L}_D(\mathbf{w}_{np}) \leq \ln\left(\frac{d}{e^{-\eta}}\right)\frac{6dL^2}{\lambda w_0 \epsilon}
\end{equation}
Note that $\hat{L}_D(\mathbf{w}_{np})-L(\mathbf{w}^*) = \hat{L}_D(\mathbf{w}_{np})-\hat{L}_D(\mathbf{w}^*)+\hat{L}_D(\mathbf{w}^*)-L(\mathbf{w}^*)$. Also, by definition, as $\mathbf{w}_{np}$ is the \textit{empirical minimizer}:
\[\hat{L}_D(\mathbf{w}_{np})+\lambda\norm{\mathbf{w}_{np}-\mathbf{w}_g}^2\leq \hat{L}_D(\mathbf{w}^*)+\lambda\norm{\mathbf{w}^*-\mathbf{w}_g}^2\]
\begin{equation}\label{eq:p2}
    \hat{L}_D(\mathbf{w}_{np})-\hat{L}_D(\mathbf{w}^*) \leq\lambda\norm{\mathbf{w}^*-\mathbf{w}_g}^2 - \lambda\norm{\mathbf{w}_{np}-\mathbf{w}_g}^2 \leq \lambda\norm{\mathbf{w}^*-\mathbf{w}_g}^2
\end{equation}
Recalling that $\lambda\leq\frac{1}{\Omega(w^*)w_0}$ we obtain:
\begin{equation}\label{eq:p3}
    \hat{L}_D(\mathbf{w}_{np})-\hat{L}_D(\mathbf{w}^*) \leq \frac{1}{w_0}
\end{equation}
Following~\cite{kuzborskij2013stability}, we then bound $\hat{L}(\mathbf{w}^*)-L(\mathbf{w}^*)$ using Bernstein's inequality to concentrate the empirical risk around its mean:
\begin{equation}\label{eq:p4}
\hat{L}_D(\mathbf{w}^*)-L(\mathbf{w}^*) \leq\sqrt{\frac{2\eta L(\mathbf{w}^*)}{w_0}}+ \frac{ 1.5M \eta}{b_0}
\end{equation}

Combining (\ref{eq:p1}), (\ref{eq:p3}) and (\ref{eq:p4}) we obtain the result.



\end{proof}
